ChatGPT for Code Refactoring: Analyzing Topics, Interaction, and Effective Prompts

Large Language Models (LLMs), such as ChatGPT, have become widely popular and widely used in various software engineering tasks such as refactoring, testing, code review, and program comprehension. Although recent studies have examined the effectiveness of LLMs in recommending and suggesting refactoring, there is a limited understanding of how developers express their refactoring needs when interacting with ChatGPT. In this paper, our goal is to explore interactions related to refactoring between developers and ChatGPT to better understand how developers identify areas for improvement in code, and how ChatGPT addresses developers' needs. Our approach involves text mining 715 refactoring-related interactions from 29,778 ChatGPT prompts and responses, as well as the analysis of developers' explicit refactoring intentions.

==> Tables/RQ1_Generic_Patterns.tex <==

\begin{table}
\centering
%\fontsize{14}{16}\selectfont
\caption{List of refactoring documentation in DevGPT (`*' captures the extension of the keyword).}
\label{Table:GeneralPatterns}
%\vspace{-.3cm}
%\begin{sideways}
\small
\begin{adjustbox}{width=0.5\textwidth,center}
%\begin{adjustbox}{width=0.8\columnwidth,totalheight=\textwidth,keepaspectratio}
%\begin{tcolorbox}[tab2,tabularx={X|X|X|X|X},,title=Potential Candidate Self-Affirmed Refactoring Patterns,boxrule=0.5pt]

\begin{tabular}{lllllll}
\toprule
\textbf{Patterns}\\
\midrule
Add* & Chang* & Chang* the name & Cleanup  & Clean* up \\
Code clarity & Code clean* & Code organization & Code review  &  Clean code \\
Creat*  & Customiz* & Easier to maintain & Encapsulat* & Enhanc*  \\
Extend* & Extract* & Fix* & Inlin* & Improv* \\
Improv* code quality & Introduc* & Merg* & Modif* & Modulariz* \\
 Migrat* & Mov* & Organiz* & Polish* & Reduc* \\
Refactor* & Refin* &  Remov* & Remov* redundant code & Renam*\\
Remov* unused dependencies  & Reorganiz* & Replac* & Restructur* & Rework* \\
Rewrit* & Simplif* & Split* \\

 \hline
       
%\end{tcolorbox}
\end{tabular}
\end{adjustbox}
%\end{sideways}
\vspace{-.2cm}
\end{table} 

%(1) Add* & (2) Chang* &  (3)  Chang* the name \\
%(4) Clean* up code & (5) Cleanup  & (6) Code clean  \\ 
%(7) Code optimization & (8) Creat*  &  (9) Extend*    \\
%(10) Extract*  & (11) Fix*  & (12) Fix code style \\
%(13) Improv*  & (14) Improve code quality   & (15) Inlin  \\
%  (16) Introduc*  &  (17) Merg* & (18) Mov* \\
%(19) Pull up & (20) Push down & (21) Repackag \\
%(22) Redesign & (23)  Reduc* & (24) Refactor \\ 
%(25) Refin* & (26) Remov*  & (27) Renam \\
%(28) Reorganiz & (29) Replac* &  (30) Restructur*  \\
%(31) Rewrit* & (32) Simplify code & (33) Split \\




\begin{comment}
\begin{table*}[h]
\centering
%\fontsize{14}{16}\selectfont
\caption{Patterns detected across issues that are associated with refactoring operations.}
\label{Table:GeneralPatterns}
%\begin{sideways}
\small
%\begin{adjustbox}{width=1.0\textwidth,center}
\begin{adjustbox}{width=1.0\textwidth,totalheight=\textwidth,keepaspectratio}
%\begin{tcolorbox}[tab2,tabularx={X|X|X|X|X},,title=Potential Candidate Self-Affirmed Refactoring Patterns,boxrule=0.5pt]

\begin{tabular}{lllll}
\toprule
\textbf{Patterns}\\
\midrule
(1) Add* & (20) Chang* & (40) CleanUp  & (59) Cleanup code &  (79) Replace it with \\ 
(2) Clean* up & (21) Clean-up & (41) Creat* & (60) Decompos* & (80)  Encapsulat*  \\ 
(3) Enhanc*  & (22) Extend* & (42) Extract* & (61) Factor* Out & (81) Fix*   \\ 
(4) Improv* & (23) Inlin* & (43) Introduc* & (62) Merg* & (82) Migrat*  \\ 
(5) Modif*  & (24) Modulariz* &  (44) Mov* & (63) Organiz* & (83) Clean* up code  \\ 
(6) Pull* Up  & (25) PullUp  & (45) Push Down & (64) PushDown & (84) Repackag*   \\ 
 (7) Re packag* & (26) Re-packag* & (46) Redesign*  & (65) Re-design* & (85) Reduc*  \\ 
(8) Refactor* & (27) Refin*  & (47) Reformat* & (66) Remov*  & (86) Renam*   \\ 
(9) Reorder* & (28) Reorganiz* & (48) Re-organiz*  & (67) Replac*  & (87) Simplify code   \\ 
(10) Restructur* & (29) Rework* & (49) Rewrit*  & (68) Re-writ* & (88) Rewrot*    \\ 
(11) Simplif* & (30) Split* & (50) Easier to maintain & (69) Code refactor*   & (89) Fix code style    \\ 
(12) Code cleanup   & (31) Code clean & (51) Chang* package & (70) Code clean up & (90) Less code    \\ 
          (13) Code rewrit*  & (32) Chang* the name  & (52) Code review & (71) Chang* name & (91) Improv* consistency \\
               (14) Minor refactor* &  (33) More refactor* &  (53) Customiz* &  (72) Code optimization & (92) Improv* code quality \\ 
         (15) Refactor* code & (34) Fix nam*  &   (54) Refactor out  & (73) Code formatting  & (93) Get rid of\\ 
         (16) Small refactor* &  (35) Some refactor* & (55) Fix* Regression  &  (74)  Code improvement &  (94) Code style \\ 
        (17) Remov* redundant  & (36) Remov* unneeded code   & (56) Remov* redundant code & (75) Remov* dependency & (95) Renam* package \\ 
          (18) Restructur* package & (37) Restructur* code & (57) Remov* unused   &  (76) Simpler nam* & (96) customis  \\ 
         (19) Beautify* & (38) Code clarity & (58) Code quality &  (78) Remov* unneeded code &  
              \\ \hline
       
%\end{tcolorbox}
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table*} 



\begin{table*}
\centering
%\fontsize{14}{16}\selectfont
\caption{Patterns detected across issues that are associated with refactoring operations and the keyword `refactor'.}
\label{Table:GeneralPatterns}
%\begin{sideways}
\small
%\begin{adjustbox}{width=1.0\textwidth,center}
\begin{adjustbox}{width=1.0\textwidth,totalheight=\textwidth,keepaspectratio}
%\begin{tcolorbox}[tab2,tabularx={X|X|X|X|X},,title=Potential Candidate Self-Affirmed Refactoring Patterns,boxrule=0.5pt]

\begin{tabular}{llllll}
\toprule
\textbf{Patterns}\\
\midrule
(1) Add* & (4) Chang* & (7) CleanUp  & (10) Clean* up code & (13) Merg* &  (16) Fix* \\ 
(2) Improv* & (5) Extend* & (8) Creat* & (11) Remov*  & (14) Refin* & (17) Rewrit*    \\ 
(3)  Reduc* &  (6) Extract* & (9) Replac* & (12) Split* & (15) Introduc* & (18) Mov* \\ \hline
       
%\end{tcolorbox}
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table*} 
\end{comment}

==> Tables/RQ2_Specific_Patterns.tex <==
\begin{table}
\fontsize{6.8}{6.8}\selectfont
%\tabcolsep=0.15cm
\begin{center}
\caption{Refactoring patterns per categories.}
\label{Table:TopSpecificKeywords}
%\vspace{-.3cm}
%\begin{adjustbox}{width=\columnwidth,center}
%\begin{adjustbox}{width=0.7\textwidth,center}
%\begin{adjustbox}{width=0.8\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lll}

\toprule
\textbf{Internal QA (\%)} &
\textbf{External QA  (\%)} &
\textbf{Code Smell  (\%)} \\
         \midrule 
    
  Dependency (25.33\%)    & Readability (22.13\%) &  Code smell (91\%)  \\ 
   Inheritance (25\%)     &  Usability (16.19\%)    &   Long method (6\%) \\ 
   Composition (14.16\%)      &  Performance (10.25\%)  & Duplicate code (3\%) \\ 
    Abstraction (12.16\%)   & Maintainability (8.32\%)    &   \\ 
   Coupling (10\%)  & Flexibility (8.32\%)   &  \\
   Encapsulation (8.83\%)   &  Reusability (7.28\%)   &  \\
   Polymorphism (3\%) &  Accessibility (7.28\%)   & \\
   Complexity (1.5\%)  &  Modularity (4.6\%)   & \\
     & Extensibility (3.86\%)  &  \\
      & Correctness (1.78\%)  & \\ 
         & Manageability (1.48\%) & \\
             & Robustness (1.48\%)  & \\
     & Compatibility (1.33\%)   &  \\
    &   Scalability (1.18\%) & \\
    & Configurability (0.89\%)   &  \\
        & Simplicity (0.89\%) & \\
    & Reliability (0.89\%) & \\
    & Productivity (0.89\%) & \\
    & Adaptability (0.59\%)  & \\
    & Understandability (0.29\%) & \\

    
        \bottomrule
\end{tabular} 
%\end{adjustbox}
\end{center}
%\vspace{-.6cm}
\end{table}

% \begin{table}
% \fontsize{6.8}{6.8}\selectfont
% %\tabcolsep=0.15cm
% \begin{center}
% \caption{Summary of refactoring patterns, clustered by refactoring related categories \eman{Anush results }.
% } 
% \label{Table:TopSpecificKeywords}
% %\begin{adjustbox}{width=\columnwidth,center}
% %\begin{adjustbox}{width=0.7\textwidth,center}
% %\begin{adjustbox}{width=0.8\textheight,totalheight=\textwidth,keepaspectratio}
% \begin{tabular}{lll}

% \toprule
% \textbf{Internal QA (\%)} &
% \textbf{External QA  (\%)} &
% \textbf{Code Smell  (\%)} \\
%          \midrule 
    
%   Complexity (64.19\%)    & Functionality (29.18\%) &  Data class (45.62\%)  \\ 
%    Design size (13.63\%)     &  Performance (25.43\%)    &   Long method (34.51\%) \\ 
%    Abstraction (7.74\%)      &  Flexibility (9.72\%)  & Duplicate code (8.37\%) \\ 
%     Composition (7.40\%)   & Compatibility (9.25\%)    & Dead code (6.01\%) \\ 
%    Inheritance (2.52\%)  & Accuracy (6.79\%)   &  Switch statement (5.46\%)\\
%    Encapsulation (2.13\%)   &  Efficiency (6.08\%)   &  \\
%    Coupling (1.40\%) &  Simplicity (5.93\%)   & \\
%    Polymorphism (0.56\%)  &  Readability (5.69\%)   & \\
%    Cohesion (0.39\%)  & Effectiveness (4.42\%)  &  \\
%       & Stability (3.73\%)  & \\ 
%          & Maintainability (3.49\%) & \\
%              & Robustness (3.22\%)  & \\
%      &  Reliability (2.25\%)   &  \\
%     &   Usability  (2.20\%) & \\
%     & Scalability (2.14\%)   &  \\
%         & Accessibility (1.81\%) & \\
%     & Correctness (1.73\%) & \\
%     & Reusability (1.39\%) & \\
%     & Productivity (1.17\%)  & \\
%     & Extensibility (0.85\%) & \\
% & Interoperability (0.78\%) & \\
% & Adaptability (0.52\%) & \\
% & Modularity (0.46\%) & \\
% & Reproducibility (0.35\%) & \\
% & Traceability (0.16\%) & \\
% & Testability (0.14\%) & \\
% & Manageability (0.13\%) & \\
% & Configurability (0.03\%) & \\

%         \bottomrule
% \end{tabular} 
% %\end{adjustbox}
% \end{center}
% \vspace{-.3cm}
% \end{table}




\begin{comment}
\begin{table}[H]
%\fontsize{7.5}{8}\selectfont
%\tabcolsep=0.15cm
\begin{center}
\caption{Summary of refactoring patterns, clustered by refactoring related categories (refactoring commits).
}
\label{Table:TopSpecificKeywords}
%\begin{adjustbox}{width=\columnwidth,center}
%\begin{adjustbox}{width=0.7\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lll}

\toprule
\textbf{Internal QA} &
\textbf{External QA} &
\textbf{Code Smell} \\
         \midrule 
    Inheritance & Functionality & Duplicate Code \\ 
    Abstraction & Performance & Dead Code  \\ 
    Complexity & Compatibility &  Redundancy  \\ 
    Composition  & Readability & Useless class \\ 
    Coupling & Stability & Code style  \\ 
    Encapsulation & Usability &  \\
    Design Size  & Flexibility &  \\
    Polymorphism & Extensibility  &  \\
    Messaging  & Accuracy  & \\ 
    Concern Separation & Accessibility & \\ 
    Dependency & Robustness &  \\
    & Reusability & \\
    & Testability & \\ 
    & Correctness & \\
    & Scalability & \\
    & Configurability & \\
    & Reliability & \\
    & Modularity &  \\
    & Maintainability & \\
    & Fault-tolerance & \\
    & Repeatability & \\
    &  Effectiveness & \\
    & Modifiability & \\
   & Manageability & \\
        \bottomrule
\end{tabular} 
%\end{adjustbox}

\end{center}
\end{table}


\begin{table}[H]
%\fontsize{7.5}{8}\selectfont
%\tabcolsep=0.15cm
\begin{center}
\caption{Summary of refactoring patterns, clustered by refactoring related categories (refactoring commits and the keyword `refactor' in title and categories in title).
}
\label{Table:TopSpecificKeywords}
%\begin{adjustbox}{width=\columnwidth,center}
%\begin{adjustbox}{width=0.7\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lll}

\toprule
\textbf{Internal QA} &
\textbf{External QA} &
\textbf{Code Smell} \\
         \midrule 
    Inheritance & Functionality & Duplicate Code \\ 
    Dependency & Performance &  \\ 
    & Compatibility &    \\ 
      & Stability &  \\ 
     & Usability &   \\ 
     & Flexibility &  \\
    & Extensibility &  \\
     &  Testability &  \\
      & Configurability  & \\ 
     & Modularity & \\ 
     & Manageability &  \\

        \bottomrule
\end{tabular} 
%\end{adjustbox}

\end{center}
\end{table}

\end{comment}


